Decentralized Strongly-Convex Optimization with Affine Constraints: Primal and Dual Approaches

Decentralized optimization is a common paradigm used in distributed signal processing and sensing as well as privacy-preserving and large-scale machine learning. It is assumed that several computational entities locally hold objective functions and are connected by a network. The agents aim to commonly minimize the sum of the local objectives subject by making gradient updates and exchanging information with their immediate neighbors. Theory of decentralized optimization is pretty well-developed in the literature. In particular, it includes lower bounds and optimal algorithms. In this paper, we assume that along with an objective, each node also holds affine constraints. We discuss several primal and dual approaches to decentralized optimization problem with affine constraints.

==> bilinear_saddle_general.tex <==
\section{Bilinear saddle with composite}

Consider problem
\begin{align*}
   \min_{\bx}~ \sum_{i=1}^m {f_i(x)} \\
    &\text{s.t. } B_0x = 0.
\end{align*}
where $\bx = (x_1^\top, \ldots, x_m^\top)^\top$, $\by = (y_1^\top, \ldots, y_m^\top)^\top$. Introduce $F(\bx) = \sum_{i=1}^m f_i(x_i),~ G(\by) = \sum_{i=1}^m g_i(y_i)$, $\mB = \text{diag}(B_1, \ldots, B_m)$. Also introduce a Laplacian $W$ and communication matrices $\mWx = W\otimes I_{d_x},~ \mWy = W\otimes I_{d_y}$. We have
\begin{align*}
    \min_{\bx, \bu} \max_{\by, \bz} \cbraces{F(\bx) - G(\by) + \angles{\by, \mB\bx} + \gamma_x\angles{\bz, \mWx\bx} + \gamma_y\angles{\bu, \mWy\by}}
\end{align*}
Or, equivalently,
\begin{align*}
    \min_{\bx, \bu} \max_{\by, \bz}~~ F(\bx) - G(\by) + 
    \angles{
    \begin{pmatrix} \by \\ \bz \end{pmatrix},
    \begin{pmatrix} \mB & \gamma_y\mWy \\ \gamma_x\mWx & \mathbf{0} \end{pmatrix}
    \begin{pmatrix} \bx \\ \bu \end{pmatrix}
    }.
\end{align*}
Denote $\mA = \begin{pmatrix} \mB & \gamma_y\mWy \\ \gamma_x\mWx & \mathbf{0} \end{pmatrix}$. Let us estimate the condition number of $\mA\mA^\top$.
\begin{align*}
    \mA\mA^T =
    \begin{pmatrix}
        \mB\mB^\top + \gamma_y^2 \mWy^2 & \gamma_x\mB\mWx \\
        \gamma_x\mWx\mB^\top & \gamma_x^2 \mWx^2
    \end{pmatrix}
\end{align*}

We consider a simplified case $B_1 = \ldots = B_m$. Then $\mB = \mI_m\otimes B_1$. To compute the eigenvalues of $\mA$, let us first diagonalize its block elements. Namely, consider singular value decomposition $B_1 = U_1\Lambda_{B_1} V_1^\top$, where $U_1\in\R^{d_y\times d_y}$ and $V_1\in\R^{d_x\times d_y}$ are orthogonal matrices and $\Lambda_{B_1}\in\R^{d_y\times d_y}$ is a diagonal matrix with singular values of $B_1$ at diagonal. Also let $W = S \Lambda_W S^T$, where $S\in\R^{m\times m}$ is an orthogonal matrix. We have
\begin{align*}
    &\begin{pmatrix}
        S^T\otimes U_1^\top & \mathbf{0} \\
        \mathbf{0} & S^T\otimes V_1^\top
    \end{pmatrix}
    \begin{pmatrix}
        \mB\mB^\top + \gamma_y^2 \mWy^2 & \gamma_x\mB\mWx \\
        \gamma_x\mWx\mB^\top & \gamma_x^2 \mWx^2
    \end{pmatrix}
    \begin{pmatrix}
        S\otimes U_1 & \mathbf{0} \\
        \mathbf{0} & S\otimes V_1
    \end{pmatrix} \\
    &= \begin{pmatrix}
        (S^\top S)\otimes (U_1^\top B_1 B_1^\top U_1) + \gamma_y^2 (S^\top W^2 S)\otimes (U_1^\top U_1) & \gamma_x (S^\top W S)\otimes (U_1^\top B_1 V_1) \\
        \gamma_x (S^T W S)\otimes (V_1^\top B_1^\top U_1) & \gamma_x^2 (S^\top W S)\otimes (V_1^\top V_1)
    \end{pmatrix} \\
    &= \begin{pmatrix}
        \mI_m\otimes \Lambda_{B_1}^2 + \gamma_y^2 \Lambda_W^2\otimes \mI_{d_y} & \gamma_x \Lambda_W\otimes \Lambda_{B_1} \\
        \gamma_x \Lambda_W\otimes \Lambda_{B_1} & \gamma_x^2 \Lambda_W^2\otimes \mI_{d_y}
    \end{pmatrix} = \mC
\end{align*}
Now let calculate the eigenvalues of $\mC$ using Schur complement.
\begin{align*}
    \det(\mC &- \lambda\mI_{2md_y}) = \det(\gamma_x\Lambda_W^2\otimes \mI_{d_y} - \lambda\mI_{md_r})\cdot \det(\mD),
\end{align*}
where 
\begin{align*}
    \mD = \mI_m\otimes\Lambda_{B_1}^2 + \gamma_y^2 \Lambda_W^2\otimes\mI_{d_y} - \lambda\mI_{md_y} - \gamma_x^2 (\Lambda_W\otimes\Lambda_{B_1})(\gamma_x^2 \Lambda_W^2\otimes \mI_{d_y} - \lambda\mI_{md_y})^{-1}(\Lambda_W\otimes\Lambda_{B_1}).
\end{align*}
Let $\Lambda_{B_1} = \text{diag}(\beta_1, \ldots, \beta_{d_y}),~ \Lambda_W = \text{diag}(w_1, \ldots, w_m)$. Then $\mD$ is a diagonal matrix with elements 
\begin{align*}
    \eta(\lambda, w_i^2, \beta_j^2) = \beta_j^2 + \gamma_y^2 w_i^2 - \lambda - \gamma_x^2\cdot \frac{w_i^2 \beta_j^2}{\gamma_x^2 w_i^2 - \lambda},~ i = 1, \ldots, m;~ j = 1, \ldots, d_y.
\end{align*}
We have $\eta(\lambda, w_i, \beta_j) = 0$ when
\begin{align*}
    \lambda^{\pm}(w_i^2, \beta_j^2) = \frac{1}{2}\cbraces{\beta_j^2 + (\gamma_x^2 + \gamma_y^2)w_i^2 \pm \sqrt{\beta_j^4 + (\gamma_x^2 - \gamma_y^2)^2 w_i^4 + 2\beta_j^2w_i^2(\gamma_x^2 + \gamma_y^2)}}
\end{align*}
We need to find the maximum and minimum \textit{nonzero} items among $\lambda^{\pm}(w_i^2, \beta_j^2)$. Firstly, note that $\lambda^+(w^2, \beta^2)$ increases both in $w^2$ and $\beta^2$. Therefore (when $\gamma_x = \gamma_y = \gamma$),
\begin{align*}
    \lambda_{\max} = \lambda^+(w_{\max}^2, \beta_{\max}^2) = \frac{1}{2}\cbraces{\beta_{\max}^2 + 2\gamma^2 w_{\max}^2 + \sqrt{\beta_{\max}^4 + 4\beta_{\max}^2\gamma^2 w_{\max}^2}}\leq \beta_{\max}^2 + 2\gamma^2 w_{\max}^2.
\end{align*}
Secondly, note that $\lambda^-(w^2, \beta^2)$ increases both in $w^2$ and $\beta^2$.
\begin{align*}
    &\frac{d\lambda^-}{d(\beta^2)} = \frac{1}{2} - \frac{1}{2}\cdot \frac{\beta^2}{\sqrt{\beta^4 + (\gamma_x^2 - \gamma_y^2)^2 w^4 + 2\beta^2 w^2(\gamma_x^2 + \gamma_y^2)}} > 0, \\
    &\frac{d\lambda^-}{d(w^2)} = \frac{1}{2}(\gamma_x^2 + \gamma_y^2) - \frac{1}{2}\cdot \frac{w^2 (\gamma_x^2 - \gamma_y^2)^2 + \beta^2(\gamma_x^2 + \gamma_y^2)}{\sqrt{\beta^4 + (\gamma_x^2 - \gamma_y^2)^2 + 2\beta^2 w^2 (\gamma_x^2 + \gamma_y^2)}} > 0.
\end{align*}
The minimal $\lambda$ is attained either at $w_i = 0$ or $w_i = w_{\min}^+$:
\begin{align*}
    \lambda_{\min}^+ = \min\braces{\lambda^+(\beta_{\min}, 0), \lambda^-(\beta_{\min}, w_{\min}^+)} = \min\braces{\beta_{\min}^2, \beta_{\min}^2 + 2\gamma^2 (w_{\min}^+)^2 - \sqrt{\beta_{\min}^4 + 4\beta_{\min}^2 \gamma^2 (w_{\min}^+)^2}}.
\end{align*}
The optimal value of $\gamma$ is $(\gamma^*)^2 = \dfrac{2\beta_{\min}^2}{(w_{\min}^+)^2}$, and we have $\chi(\mD) \sim \chi^2(B_1) + \chi^2(W)$.


==> commands.tex <==
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{mathtools}
\mathtoolsset{showonlyrefs}
\mathtoolsset{showmanualtags}
\usepackage{amsthm}
\usepackage{xcolor}
\usepackage{tabularx}
\usepackage{bbm}
\usepackage{todonotes}
\usepackage{amsmath}
\usepackage{makecell}
\usepackage{subcaption}


\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand{\dmitry}[1]{\todo[inline]{\footnotesize Dmitry: #1}}
\newcommand{\peter}[1]{\todo[inline]{\footnotesize Peter: #1}}
\newcommand{\adil}[1]{\todo[inline]{\footnotesize Adil: #1}}
\newcommand{\as}[1]{{\color{green} #1}}
\newcommand{\asnote}[1]{\todo[color=green!]{#1}}

\allowdisplaybreaks[1]



\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}

\newcommand{\AG}{\mathrm{AG}}

\newcommand{\prox}{\mathrm{prox}}
\newcommand{\range}{\mathrm{range}}
\newcommand{\Comp}{\mathrm{Comp}}
\newcommand{\Comm}{\mathrm{Comm}}
\newcommand{\Span}{\mathrm{Span}}
\newcommand{\Sp}{\mathrm{Sp}}

\newcommand{\bg}{\mathrm{D}}

\newcommand{\R}{\mathbb{R}}

\def\<#1,#2>{\langle #1,#2\rangle}

\newcommand{\Dotprod}[1]{\left\langle#1\right\rangle}


\newcommand{\norm}[1]{\|#1\|}
\newcommand{\sqn}[1]{\norm{#1}^2}
\newcommand{\Norm}[1]{\left\|#1\right\|}
\newcommand{\sqN}[1]{\Norm{#1}^2}
\newcommand{\vect}[1]{\begin{bmatrix*}[l]#1\end{bmatrix*}}

\newcommand{\cR}{\mathcal{R}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\sX}{{\mathsf E}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\Lag}{\mathcal{L}}
\newcommand{\mA}{\mathbf{A}}
\newcommand{\mW}{\mathbf{W}}
\newcommand{\mL}{\mathbf{L}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mP}{\mathbf{P}}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\mWp}{\mathbf{W}^{\dagger}}
\newcommand{\sqnw}[1]{\sqn{#1}_{\mWp}}
\newcommand{\eqdef}{\coloneqq}
\DeclareMathOperator*{\argmin}{arg\,min}

